Zero-shot Building Age Classification from Facade Image Using GPT-4

A building's age of construction is crucial for supporting many geospatial applications. Much current research focuses on estimating building age from facade images using deep learning. However, building an accurate deep learning model requires a considerable amount of labelled training data, and the trained models often have geographical constraints. Recently, large pre-trained vision language models (VLMs) such as GPT-4 Vision, which demonstrate significant generalisation capabilities, have emerged as potential training-free tools for dealing with specific vision tasks, but their applicability and reliability for building information remain unexplored. In this study, a zero-shot building age classifier for facade images is developed using prompts that include logical instructions. Taking London as a test case, we introduce a new dataset, FI-London, comprising facade images and building age epochs. Although the training-free classifier achieved a modest accuracy of 39.69%, the mean absolute error of 0.85 decades indicates that the model can predict building age epochs successfully albeit with a small bias. The ensuing discussion reveals that the classifier struggles to predict the age of very old buildings and is challenged by fine-grained predictions within 2 decades. Overall, the classifier utilising GPT-4 Vision is capable of predicting the rough age epoch of a building from a single facade image without any training.

==> Equotions/F1.tex <==
\begin{equation}
\label{equ:weighted_F1}
\begin{split}
\text{F1 Score} &= 2 \times \frac{\text{Precision} \times \text{Recall}}{\text{Precision} + \text{Recall}} \\
&= 2 \times \frac{\text{TP}/(\text{TP} + \text{FP})\times \text{TP}/(\text{TP} + \text{FN})}{\text{TP}/(\text{TP} + \text{FP}) + \text{TP}/(\text{TP} + \text{FN})}
&=
\end{split}
\end{equation}

%\begin{tabbing} 
%where \hspace{0.6cm} \= TP = True Positive Sample(s)\\
%\> FP = False Positive Sample(s)\\
%\> FN = False Negative Sample(s)
%\end{tabbing}

% \begin{equation}
% \text{F1} = \sum_{c \in C} w_c \times \text{F1}_c
% \end{equation}

% F_1 = \frac{2 \times \text{Precision} \times \text{Recall}}{\text{Precision} + \text{Recall}}

==> Equotions/Precision.tex <==
\begin{equation}\label{equ}
\text{Precision} = \frac{\text{TP}}{\text{TP} + \text{FP}}
\end{equation}


==> Equotions/Recall.tex <==
\begin{equation}
\text{Recall} = \frac{\text{TP}}{\text{TP} + \text{FN}}
\end{equation}


==> Equotions/Task.tex <==
\begin{equation}
AE = \text{Top@}k_{c \in C} \, P(c | D)
\end{equation}

\begin{tabbing} 
where \hspace{0.6cm} \= $AE$ = Age Epoch(s)\\
\> Top@$5$ = $5$ maximum probability categories\\
\> $C$ = the set of 15 building age epoch categories
\end{tabbing}


==> Equotions/Top_k.tex <==
\begin{equation}\label{equ:1}
\text{Top@$k$ Accuracy} = \frac{1}{N} \sum_{i=1}^{N} \mathbf{1}(y_i \in P_k(x_i))
\end{equation}



==> Tables/Topk_n_WeightedF1.tex <==
\begin{table}[b]
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{c|ccc|c}
\toprule[2pt]
\multirow[m]{2}{*}{Age Epoch}&\multicolumn{3}{c|}{Accuracy}&\multirow[m]{2}{*}{Weighted F1}\\
 &Top@1(\%)&Top@3(\%)&Top@5(\%)& \\
\midrule
$>$2020&66.67&100.00&100.00&0.33 \\
2000-2019&23.08&84.62&92.31&0.20 \\
1980-1999&10.00&100.00&100.00&0.12 \\
1960-1979&50.00&87.50&100.00&0.36 \\
1940-1959&7.14&64.29&100.00&0.13 \\
1920-1939&68.75&75.00&93.75&0.51 \\
1900-1919&40.00&100.00&100.00&0.32 \\
1880-1899&30.00&90.00&90.00&0.27 \\
1860-1879&16.67&66.67&100.00&0.29 \\
1840-1859&0.00&16.67&66.67&0.00 \\
1820-1839&0.00&37.50&37.50&0.00 \\
1800-1819&75.00&75.00&75.00&0.36 \\
1750-1799&0.00&77.78&88.89&0.00 \\
1700-1749&14.29&14.29&14.29&0.25 \\
$<$1700&0.00&0.00&0.00&0.00 \\
\midrule
Total&28.24&70.99&83.21&0.23 \\
\bottomrule[2pt]
\end{tabular}
}
\caption{Performance of zero-shot classifier on FI-London}
\label{tab:perfomance}

\end{table}
